Rigorous Computation of Linear Response for Intermittent Maps

We present a rigorous numerical scheme for the approximation of the linear response of the invariant density of a map with an indifferent fixed point, with explicit and computed estimates for the error and all the involved constants.

==> data.tex <==
% Autogenerated by LaTeXDatax.jl, will be overwritten
\pgfkeyssetvalue{/datax/α}{$0.5$}
\pgfkeyssetvalue{/datax/γ}{$0.501$}
\pgfkeyssetvalue{/datax/D0}{$2.956$}
\pgfkeyssetvalue{/datax/D}{$19.22$}
\pgfkeyssetvalue{/datax/D0calc}{$[2.78189, 2.79035]$}
\pgfkeyssetvalue{/datax/delta_k}{$2.146 \cdot 10^{-12}$}
\pgfkeyssetvalue{/datax/Lemma31const}{$78.01$}
\pgfkeyssetvalue{/datax/Lemma31contract}{$0.002062$}
\pgfkeyssetvalue{/datax/hc1bound}{$377.9$}
\pgfkeyssetvalue{/datax/herror}{$7.662$}
\pgfkeyssetvalue{/datax/herror1}{$1.794$}
\pgfkeyssetvalue{/datax/herror2}{$5.868$}
\pgfkeyssetvalue{/datax/AppendixLM}{$6.911$}
\pgfkeyssetvalue{/datax/eta}{$9.537 \cdot 10^{-07}$}
\pgfkeyssetvalue{/datax/lstar}{$99$}
\pgfkeyssetvalue{/datax/gamma_const}{$1.418$}
\pgfkeyssetvalue{/datax/N}{$1048576$}
\pgfkeyssetvalue{/datax/branches}{$200$}
\pgfkeyssetvalue{/datax/a_n}{$1500$}
\pgfkeyssetvalue{/datax/b_n}{$10$}
\pgfkeyssetvalue{/datax/jstar}{$586$}
\pgfkeyssetvalue{/datax/a_ω}{$0.6227$}
\pgfkeyssetvalue{/datax/b_ω}{$1817$}
\pgfkeyssetvalue{/datax/g_ω_prime}{$0.0114$}
\pgfkeyssetvalue{/datax/g_ω_bad_branches}{$0.05687$}
\pgfkeyssetvalue{/datax/g_ω_tail}{$1.14 \cdot 10^{-05}$}
\pgfkeyssetvalue{/datax/C_1}{$0.88$}
\pgfkeyssetvalue{/datax/C_2}{$16.77$}
\pgfkeyssetvalue{/datax/C_3}{$9.022$}
\pgfkeyssetvalue{/datax/C_4}{$9.475$}
\pgfkeyssetvalue{/datax/C_5}{$1.091$}
\pgfkeyssetvalue{/datax/C_6}{$1.227$}
\pgfkeyssetvalue{/datax/C_7}{$0.1534$}
\pgfkeyssetvalue{/datax/C_10}{$50.58$}
\pgfkeyssetvalue{/datax/C_11}{$1739$}
\pgfkeyssetvalue{/datax/C_12}{$1232$}
\pgfkeyssetvalue{/datax/cu1}{$1$}
\pgfkeyssetvalue{/datax/cu2}{$1$}
\pgfkeyssetvalue{/datax/cu3}{$1$}
\pgfkeyssetvalue{/datax/cu4}{$1$}
\pgfkeyssetvalue{/datax/cu5}{$1$}
\pgfkeyssetvalue{/datax/cu6}{$1$}
\pgfkeyssetvalue{/datax/cu7}{$1$}
\pgfkeyssetvalue{/datax/cu8}{$1$}
\pgfkeyssetvalue{/datax/cu9}{$1$}
\pgfkeyssetvalue{/datax/cu10}{$0.09782$}
\pgfkeyssetvalue{/datax/cu11}{$0.02349$}
\pgfkeyssetvalue{/datax/cu12}{$0.005539$}
\pgfkeyssetvalue{/datax/lemmaB4_λ1}{$0.25$}
\pgfkeyssetvalue{/datax/lemmaB4_A}{$2.491$}
\pgfkeyssetvalue{/datax/lemmaB4_B}{$49.22$}
\pgfkeyssetvalue{/datax/lemmaB4_δ}{$9.537 \cdot 10^{-07}$}
\pgfkeyssetvalue{/datax/lemmaB4_K}{$30.91$}
\pgfkeyssetvalue{/datax/lemmaB4_P}{$2.875$}
\pgfkeyssetvalue{/datax/lemmaB4_M}{$7.452$}
\pgfkeyssetvalue{/datax/f_weak}{$8.52$}
\pgfkeyssetvalue{/datax/f_strong}{$419.4$}
\pgfkeyssetvalue{/datax/f_inf}{$1.373$}
\pgfkeyssetvalue{/datax/f_var}{$0.7456$}
\pgfkeyssetvalue{/datax/Nstar}{$1000$}
\pgfkeyssetvalue{/datax/b_ωNstar}{$52.88$}
\pgfkeyssetvalue{/datax/AppendixZ}{$10.1$}
\pgfkeyssetvalue{/datax/AppendixM}{$2.491$}
\pgfkeyssetvalue{/datax/AppendixB}{$0.7456$}
\pgfkeyssetvalue{/datax/AppendixM2}{$6.206$}
\pgfkeyssetvalue{/datax/AppendixCstar}{$7.452$}
\pgfkeyssetvalue{/datax/AppendixC2}{$49.85$}
\pgfkeyssetvalue{/datax/ρbv}{$0.09785$}
\pgfkeyssetvalue{/datax/ρC1}{$0.1957$}
\pgfkeyssetvalue{/datax/SMuA}{$0.002927$}
\pgfkeyssetvalue{/datax/SMuB}{$0.0182$}
\pgfkeyssetvalue{/datax/Lemma373}{$0.0001707$}
\pgfkeyssetvalue{/datax/Lemma374}{$0.0006418$}
\pgfkeyssetvalue{/datax/PB1}{$33.43$}
\pgfkeyssetvalue{/datax/PB2}{$0.00235$}
\pgfkeyssetvalue{/datax/PB3}{$1.975 \cdot 10^{4}$}
\pgfkeyssetvalue{/datax/PB4}{$62$}
\pgfkeyssetvalue{/datax/PBerror}{$1.984 \cdot 10^{4}$}
\pgfkeyssetvalue{/datax/InducedC1Contract}{$0.3647$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfkeyssetvalue{/datax/hetaC0}{$1.124$}
\pgfkeyssetvalue{/datax/hprimeetaC0}{$0.3423$}
\pgfkeyssetvalue{/datax/AppendixWb}{$0.0008494$}
\pgfkeyssetvalue{/datax/AppendixWa}{$8.067 \cdot 10^{-07}$}
\pgfkeyssetvalue{/datax/AppendixW}{$0.08417$}
\pgfkeyssetvalue{/datax/Wnorm}{$0.5098$}
\pgfkeyssetvalue{/datax/AppendixWlstarratio}{$0.01131$}
\pgfkeyssetvalue{/datax/AppendixWlstar}{$0.005768$}
\pgfkeyssetvalue{/datax/VarInterior}{$0.2563$}
\pgfkeyssetvalue{/datax/L1Interior}{$0.004301$}
\pgfkeyssetvalue{/datax/AppendixWu1}{$0.003943$}
\pgfkeyssetvalue{/datax/AppendixWu2}{$16.63$}
\pgfkeyssetvalue{/datax/ILRerror}{$16.72$}
\pgfkeyssetvalue{/datax/PB1}{$33.43$}
\pgfkeyssetvalue{/datax/hstaretaC0}{$0.2185$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfkeyssetvalue{/datax/hetastar_pb_error}{$0.007765$}
\pgfkeyssetvalue{/datax/I}{$0.001533$}
\pgfkeyssetvalue{/datax/II}{$4.603 \cdot 10^{-10}$}
\pgfkeyssetvalue{/datax/III}{$6.818 \cdot 10^{-6}$}
\pgfkeyssetvalue{/datax/IV}{$0.006225$}
\pgfkeyssetvalue{/datax/gamma_const}{$1.414$}
\pgfkeyssetvalue{/datax/SummableConst}{$5.981$}
\pgfkeyssetvalue{/datax/aomega_max}{$7107$}
\pgfkeyssetvalue{/datax/hetaprime_max}{$1$}
\pgfkeyssetvalue{/datax/gprime_tail}{$6.51 \cdot 10^{-10}$}
\pgfkeyssetvalue{/datax/heta_max}{$1.5$}
\pgfkeyssetvalue{/datax/bomega_tail}{$0.002931$}
\pgfkeyssetvalue{/datax/heta_error}{$3.833 \cdot 10^{-9}$}
\pgfkeyssetvalue{/datax/h_error_1}{$2.113 \cdot 10^{-9}$}
\pgfkeyssetvalue{/datax/h_error_2}{$1.72 \cdot 10^{-9}$}
\pgfkeyssetvalue{/datax/bomega_sum}{$1258$}
\pgfkeyssetvalue{/datax/gamma_const}{$1.414$}
\pgfkeyssetvalue{/datax/hetastar_max}{$0.5$}
\pgfkeyssetvalue{/datax/hetastar_error}{$0.0007666$}
\pgfkeyssetvalue{/datax/hstar_error_4}{$2 \cdot 10^{-289}$}
\pgfkeyssetvalue{/datax/hstar_error_3}{$3.055 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/hstar_error_2}{$9.616 \cdot 10^{-8}$}
\pgfkeyssetvalue{/datax/hstar_error_1}{$0.0007662$}
\pgfkeyssetvalue{/datax/A0Accuracy}{$10$}
\pgfkeyssetvalue{/datax/alph}{$0.125$}
\pgfkeyssetvalue{/datax/gamma}{$0.5$}
\pgfkeyssetvalue{/datax/jstar}{$1000$}
\pgfkeyssetvalue{/datax/Nstar}{$1000$}
\pgfkeyssetvalue{/datax/lstar}{$988$}
\pgfkeyssetvalue{/datax/lstarn}{$22$}
\pgfkeyssetvalue{/datax/lstarcontract}{$2.991 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/IDN}{$10$}
\pgfkeyssetvalue{/datax/WL1}{$968.7$}
\pgfkeyssetvalue{/datax/W1}{$3.046 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/W2}{$9.007 \cdot 10^{-10}$}
\pgfkeyssetvalue{/datax/C8}{$2.766$}
\pgfkeyssetvalue{/datax/D}{$1.286$}
\pgfkeyssetvalue{/datax/D0}{$0.2513$}
\pgfkeyssetvalue{/datax/C8jstarx}{$-0.02057$}
\pgfkeyssetvalue{/datax/hpbI}{$7.666 \cdot 10^{-9}$}
\pgfkeyssetvalue{/datax/hpbII}{$1.381 \cdot 10^{-9}$}
\pgfkeyssetvalue{/datax/hpb}{$9.047 \cdot 10^{-9}$}
\pgfkeyssetvalue{/datax/eta}{$9.537 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/cu1}{$1$}
\pgfkeyssetvalue{/datax/cu2}{$1$}
\pgfkeyssetvalue{/datax/cu3}{$1$}
\pgfkeyssetvalue{/datax/cu4}{$1$}
\pgfkeyssetvalue{/datax/cu5}{$1$}
\pgfkeyssetvalue{/datax/cu6}{$1$}
\pgfkeyssetvalue{/datax/cu7}{$1$}
\pgfkeyssetvalue{/datax/cu8}{$1$}
\pgfkeyssetvalue{/datax/cu9}{$1$}
\pgfkeyssetvalue{/datax/cu10}{$0.09782$}
\pgfkeyssetvalue{/datax/cu11}{$0.02349$}
\pgfkeyssetvalue{/datax/cu12}{$0.005539$}
\pgfkeyssetvalue{/datax/cc1}{$3.674$}
\pgfkeyssetvalue{/datax/cc2}{$1.254$}
\pgfkeyssetvalue{/datax/cc3}{$0.4237$}
\pgfkeyssetvalue{/datax/cc4}{$0.1427$}
\pgfkeyssetvalue{/datax/cc5}{$0.04799$}
\pgfkeyssetvalue{/datax/cc6}{$0.01613$}
\pgfkeyssetvalue{/datax/cc7}{$0.005421$}
\pgfkeyssetvalue{/datax/cc8}{$0.001821$}
\pgfkeyssetvalue{/datax/cc9}{$0.0006119$}
\pgfkeyssetvalue{/datax/cc10}{$0.0002056$}
\pgfkeyssetvalue{/datax/cc11}{$0.0007551$}
\pgfkeyssetvalue{/datax/cc12}{$0.0002577$}
\pgfkeyssetvalue{/datax/cc13}{$8.71 \cdot 10^{-5}$}
\pgfkeyssetvalue{/datax/cc14}{$2.934 \cdot 10^{-5}$}
\pgfkeyssetvalue{/datax/cc15}{$9.866 \cdot 10^{-6}$}
\pgfkeyssetvalue{/datax/cc16}{$3.316 \cdot 10^{-6}$}
\pgfkeyssetvalue{/datax/cc17}{$1.114 \cdot 10^{-6}$}
\pgfkeyssetvalue{/datax/cc18}{$3.744 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/cc19}{$1.258 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/cc20}{$4.226 \cdot 10^{-8}$}
\pgfkeyssetvalue{/datax/Lemma31Const}{$3.609$}
\pgfkeyssetvalue{/datax/L31}{$7.743 \cdot 10^{-12}$}
\pgfkeyssetvalue{/datax/Cstar}{$7.452$}
\pgfkeyssetvalue{/datax/C1N}{$4$}
\pgfkeyssetvalue{/datax/LkLC1}{$2.734 \cdot 10^{-10}$}
\pgfkeyssetvalue{/datax/LkC1contraction}{$0.1557$}
\pgfkeyssetvalue{/datax/hdeltaBV}{$1.246$}
\pgfkeyssetvalue{/datax/hdeltaC1}{$7.731$}
\pgfkeyssetvalue{/datax/hdeltaC2}{$386.6$}
\pgfkeyssetvalue{/datax/C_4}{$9.475$}
\pgfkeyssetvalue{/datax/LYerror}{$3.297 \cdot 10^{-11}$}
\pgfkeyssetvalue{/datax/Chebyshev_error}{$3.901 \cdot 10^{-12}$}
\pgfkeyssetvalue{/datax/Chebyshev_ν}{$5$}
\pgfkeyssetvalue{/datax/Chebyshev_n}{$1024$}
\pgfkeyssetvalue{/datax/partition_n}{$2^{20}$}
\pgfkeyssetvalue{/datax/V}{$7.953 \cdot 10^{5}$}
\pgfkeyssetvalue{/datax/normalised_pb}{$4.11 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/normalisedstar_pb}{$0.01501$}
\pgfkeyssetvalue{/datax/LB131}{$8.5 \cdot 10^{-7}$}
\pgfkeyssetvalue{/datax/LB132}{$3.203 \cdot 10^{-6}$}
\pgfkeyssetvalue{/datax/WprimeBound}{$1.08287 \cdot 10^{-5}$}
\pgfkeyssetvalue{/datax/gppaSum}{$0.36434$}
%For the alternative section
\pgfkeyssetvalue{/datax/Cp01}{$0.08016$}
\pgfkeyssetvalue{/datax/Cp02}{$0.1894$}
\pgfkeyssetvalue{/datax/Cp}{$0.2696$}
\pgfkeyssetvalue{/datax/TB}{$0.2513$}
\pgfkeyssetvalue{/datax/TM}{$1.503$}
\pgfkeyssetvalue{/datax/TM2}{$2.258$}
\pgfkeyssetvalue{/datax/TD}{$12.19$}
\pgfkeyssetvalue{/datax/TZ}{$1.365$}
\pgfkeyssetvalue{/datax/hDeltaBV}{$1.251$}
\pgfkeyssetvalue{/datax/hDeltaC1}{$2.825$}
\pgfkeyssetvalue{/datax/hDeltaC2}{$34.45$}
\pgfkeyssetvalue{/datax/Cstar}{$3.009$}
\pgfkeyssetvalue{/datax/Alt_h_error_2}{$0.1769$}
\pgfkeyssetvalue{/datax/Alt_h_error}{$0.1769$}
\pgfkeyssetvalue{/datax/AltPB_error}{$0.3539$}

